ACT as Human: Multimodal Large Language Model Data Annotation with Critical Thinking

Supervised learning relies on high-quality labeled data, but obtaining such data through human annotation is both expensive and time-consuming. Recent work explores using large language models (LLMs) for annotation, but LLM-generated labels still fall short of human-level quality. To address this problem, we propose the Annotation with Critical Thinking (ACT) data pipeline, where LLMs serve not only as annotators but also as judges to critically identify potential errors. Human effort is then directed towards reviewing only the most "suspicious" cases, significantly improving the human annotation efficiency. Our major contributions are as follows: (1) ACT is applicable to a wide range of domains, including natural language processing (NLP), computer vision (CV), and multimodal understanding, by leveraging multimodal-LLMs (MLLMs). (2) Through empirical studies, we derive 7 insights on how to enhance annotation quality while efficiently reducing the human cost, and then translate these findings into user-friendly guidelines. (3) We theoretically analyze how to modify the loss function so that models trained on ACT data achieve similar performance to those trained on fully human-annotated data. Our experiments show that the performance gap can be reduced to less than 2% on most benchmark datasets while saving up to 90% of human costs.

==> Figures/appendices/apx-table_of_contents.tex <==
\section*{Appendices Contents} \label{apx_toc}

% \textcolor{red}{The appendices are included in the supplementary material, which can be downloaded directly via the following link:} \textcolor{black}{\url{https://openreview.net/attachment?id=V1FlwrsseI&name=supplementary_material}.}
% \textcolor{red}{If the link does not work properly, please kindly refer to the paper's page on OpenReview to download the supplementary material as follows:}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=1\linewidth]{Figures/supp_link.png}
% \end{figure}

\textbf{A \: Supplementary Experimental Details}\label{apx_A}

\begin{enumerate}[label=\textbf{A.\arabic*.}, leftmargin=3em]
    \item Datasets
    \item Device \& Random Seed
    \item Downstream Training
\end{enumerate}

\vspace{0.2cm}

\textbf{B \: Stability Analyses} \label{apx_B}

\begin{enumerate}[label=\textbf{B.\arabic*.}, leftmargin=3em]
    \item Robustness of Annotation and Criticism Results
    \item Impact of Different Sampling Rules on Criticism
\end{enumerate}

\vspace{0.2cm}

\textbf{C \: Examples of Prompt Strategies} \label{apx_C}

\vspace{0.2cm}

\textbf{D \: Theoretical Proofs} \label{apx_D}

\begin{enumerate}[label=\textbf{D.\arabic*.}, leftmargin=3em]
    \item Proof of Proposition 5.1 – Statistical Properties of ACT Loss (Variance)
    \item Proof of Theorem 5.2 – Probabilistic Upper Bound of the Parameter Gap
\end{enumerate}

\vspace{0.2cm}

\textbf{E \: Further Details of ACT Losses} \label{apx_E}

\begin{enumerate}[label=\textbf{E.\arabic*.}, leftmargin=3em]
    \item ACT Losses with Different Sampling Rules
    \item Distributions of Transformed Errors with Different Sampling Rules
\end{enumerate}

\vspace{0.2cm}

\textbf{F \: Sensitivity Analyses of Human Budget} \label{apx_F}

\begin{enumerate}[label=\textbf{F.\arabic*.}, leftmargin=3em]
    \item AQG vs. Human Budget
    \item Downstream Performance vs. Human Budget
\end{enumerate}

\vspace{0.2cm}

\textbf{G \: Extended Discussions and Experiments} \label{apx_G}

\begin{enumerate}[label=\textbf{G.\arabic*.}, leftmargin=3em]
    \item Additional Related Works
    \item Potential Improvements of ACT
    \item Supplementary Experiments

    \begin{enumerate}
    [label=\textbf{G.3.\arabic*.}, leftmargin=3em]
        \item Comparison with CDI
        \item Comparison with Active Learning and Pseudo Labels
        \item More Challenging Tasks: Biased and Long-tail Data
        \item Analyses on Critic True Positives and False Positives
        \item Ablation of Annotator-Criticizer Selection
        \item Cost-Benefit Analysis
    \end{enumerate}

    \item Extend ACT to More Complex Tasks
    \item Ethical Considerations
    
\end{enumerate}


==> Figures/appendices/apx1-exp_details.tex <==
\section{\textbf{Supplementary Experimental Details}}\label{apx: exp_details}

\subsection{Datasets}

\begin{table}[ht]
\centering
\caption{Dataset details.}
\label{tab: apx_data}
\rowcolors{2}{gray!10}{white}
\renewcommand{\arraystretch}{1.5}
\resizebox{\linewidth}{!}{
\begin{tabular}{lclccc}
\toprule
\textbf{Dataset} & \textbf{Type} & \textbf{Description} & \textbf{\#Classes} & \textbf{Size - Train} & \textbf{Size - Test} \\
\midrule
CIFAR10             & CV   & Image classification of basic image categories.            & 10  & 50,000 & 10,000 \\
Fashion-MNIST       & CV   & Image classification of cloth items.                       & 10  & 60,000 & 10,000 \\
Stanford Cars       & CV   & Image classification of car models.                        & 196 & 8,143 & 8,040 \\
TweetEval-Emotion   & NLP  & Text emotion classification.            & 4   & 3,257 & 1,421  \\
TweetEval-Irony     & NLP  & Text rony detection.                   & 2   & 2,862 &784  \\
VQA-RAD (Close-end)            & VQA  & Question-answer pairs on radiology images.     & 2   & 940 & 262 \\
\bottomrule
\end{tabular}}
\end{table}


\begin{table}[ht]
\centering
\caption{Dataset sources and licenses retrieved from \url{https://paperswithcode.com/datasets}.}
\label{tab:dataset_sources}
\rowcolors{2}{gray!10}{white}
\renewcommand{\arraystretch}{1.5}
\resizebox{\linewidth}{!}{
\begin{tabular}{lll}
\toprule
\textbf{Dataset} & \textbf{Source} & \textbf{License} \\
\midrule
CIFAR10           & \url{https://www.cs.toronto.edu/~kriz/cifar.html} & \codebox{N/A}\\
Fashion-MNIST     & \url{https://github.com/zalandoresearch/fashion-mnist} & \codebox{MIT} \\
Stanford Cars     & \url{https://paperswithcode.com/dataset/stanford-cars} & \codebox{Custom (non-commercial)}\\
TweetEval-Emotion & \url{https://github.com/cardiffnlp/tweeteval} & \codebox{N/A}\\
TweetEval-Irony   & \url{https://github.com/cardiffnlp/tweeteval} & \codebox{N/A}\\
VQA-RAD           & \url{https://paperswithcode.com/dataset/vqa-rad} & \codebox{CC0 1.0 Universal}\\
\bottomrule
\end{tabular}}
\end{table}

\subsection{Device \& Random Seed}
All experiments are conducted with 1 to 8 NVIDIA SXM5 H100 GPUs with 80GB memories. When applicable, we set the random seed to 42 for all controllable sources of randomness.


\subsection{Downstream Training}

\textbf{Sampling} For the thresholding sampling rule, the threshold $\tau$ is determined by the quartile corresponding to the human budget proportion. Specifically, we rank the errors in descending order and set $\tau$ as the quartile value that matches the given proportion of the human budget. For the exponential weighting sampling rule, we try $\beta = 10$ or $100$ for all datasets. The mean transition parameter $\alpha$ is set in the same way as $\tau$, based on the corresponding quartile.



\textbf{ResNet18} For all datasets, we fine-tune the ResNet18 model initialized with ImageNet-pretrained weights for 10 epochs. The batch size is set to 4096 for CIFAR-10 and Fashion-MNIST, and 32 for the Stanford Cars dataset. We use the Adam optimizer for CIFAR-10 and Fashion-MNIST, while the SGD optimizer is employed for Cars, following the implementation described in \url{https://www.kaggle.com/code/archanatrivedi/resnet18-on-stanford-car-dataset}. The key hyperparameters include the learning rate, with a search space of [1$e$-2, 1$e$-3, 5$e$-4, 1$e$-4], and the power-tuning parameter for ACT losses, with values selected from [0.6, 0.7, 0.8, 0.9, 1.0] (see Appendix~\ref{apx: losses} for more details about the power-tuning parameter).

\textbf{RoBERTa}
For text classification tasks, we fine-tune the RoBERTa-base model for 5 epochs. We set the batch size to 32 and use the AdamW optimizer. The key hyperparameters include the learning rate, with a search space of [1$e$-4, 5$e$-5, 2$e$-5, 1$e$-5], and the power-tuning parameter for ACT losses, with values selected from [0.6, 0.7, 0.8, 0.9, 1.0].


\textbf{BLIP-VQA}
For VQA-RAD, we fine-tune the BLIP-VQA model initialized with the \texttt{blip-vqa-base} for 10 epochs. Since we adopt the close-ended version of VQA-RAD, where answers are limited to either “Yes” or “No”, we use these two tokens as ground truth. During both training and inference, the model is prompted to generate either “Yes” or “No” in the response token space. We evaluate the trained model by checking if the first generated response token—either 'Yes' or 'No'—matches the correct answer. We use a batch size of 32 and optimize the model using the AdamW optimizer. The key hyperparameters include the learning rate, searched over [2$e$-4, 1$e$-4, 5$e$-5, 2$e$-5], and the power-tuning parameter for ACT losses, selected from [0.6, 0.7, 0.8, 0.9, 1.0].



\clearpage

==> Figures/appendices/apx2-stability_analysis.tex <==
\section{\textbf{Stability Analyses}} \label{apx: stability}

\subsection{Robustness of Annotation and Criticism Results}
We assess the robustness of both annotation and criticism by repeating the process 5 times for each MLLM involved in our explorations. We perform the stability test on a subset of all datasets (i.e., 100 random samples per class). The results are shown in Figure \ref{fig: apx_stability_annot}, Figure \ref{fig: apx_stability_cri_bx}, and Figure \ref{fig: apx_stability_cri_wx}, respectively. We observe that the standard deviations are generally low (most within 2\%). In addition, the rank of abilities does not change after taking account of potential variations in metric values, indicating that the conclusions drawn from our explorations are robust to randomness.

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{Figures/apx_stability_annot.pdf}
    \caption{ Annotation accuracy with error bars (mean $\pm$ std). Results are presented for the CoT prompt strategy across 6 MLLM annotators.}
    \label{fig: apx_stability_annot}
\end{figure}

\begin{figure}[h!]
    \centering
    \includegraphics[width=1\linewidth]{Figures/apx_stability_cri_bx.pdf}
        \caption{Criticism ABS with error bars (mean $\pm$ std). Results are presented for the black-box CoT prompt strategy across 6 MLLM criticizers.}
    \label{fig: apx_stability_cri_bx}
\end{figure}

\begin{figure}[h!]
    \centering
    \includegraphics[width=1\linewidth]{Figures/apx_stability_cri_wx.pdf}
        \caption{Criticism ABS with error bars (mean $\pm$ std). Results are presented for the white-box naïve-logit prompt strategy across 3 MLLM criticizers.}
    \label{fig: apx_stability_cri_wx}
\end{figure}



\subsection{Impact of Different Sampling Rules on Criticism}
In Figure \ref{fig: apx_stability_sampler}, we present results computed on the full datasets using different sampling rules to evaluate the criticism ABS. The results indicate that the choice of sampling rule has minimal impact on the comparative outcomes. Therefore, the insights derived from our analyses using the thresholding rule remain consistent across other sampling methods as well.

\begin{figure}[h!]
    \centering
    \includegraphics[width=1\linewidth]{Figures/apx_stability_sampler.pdf}
    \caption{Criticism ABS with various sampling rules. Results are presented for the black-box CoT strategy across 6 MLLM criticizers.}
    \label{fig: apx_stability_sampler}
\end{figure}







==> Figures/appendices/apx3-prompts.tex <==
\section{\textbf{Examples of Prompt Strategies}}\label{apx: prompt}

Here, we present examples of prompt strategies. For annotation prompt - naïve, we include examples for all three tasks (image classification, text classification, and VQA) to provide a comprehensive illustration. For other prompt strategies, we only present examples for image classification, but they can be easily adapted to other tasks by following the same pattern as the annotation prompts.
In the following examples, \textcolor{purple}{\{purple\}} denotes inputs, while \textcolor{cyan}{[blue]} denotes outputs. Note that we require MLLMs to follow a specific output format to simplify the extraction of CoT and labels. In practice, we observe that MLLMs follow the formatting instructions well.

\begin{custombox}{Illustrations of Inputs and Outputs}

\begin{itemize}[left=0.5em]
    \item \textcolor{purple}{\{image\_data\}}, \textcolor{purple}{\{text\_data\}}, and \textcolor{purple}{\{question\}}: Images, texts, and questions from the datasets.

    \item \textcolor{purple}{\{label\_list\_with\_index\}}: A label list with indices of each label, for example, ``0: airplane, 1: automobile, 2: bird, 3: cat, 4: deer, 5: dog, 6: frog, 7: horse, 8: ship, 9: truck''.

    \item \textcolor{purple}{\{first\_label\}}: The first label in the label list, for example, ``airplane''.

    \item \textcolor{purple}{\{label\_index\}} \& \textcolor{cyan}{[label\_index]}: The label index generated by the annotator.

    \item \textcolor{cyan}{[error\_probability]} \&  \textcolor{cyan}{[error\_level]}: The error probability or level generated by the criticizer.

    \item \textcolor{purple}{\{CoT\_A\}} \& \textcolor{cyan}{[CoT\_A]}: The CoT generated by the annotator.

    \item \textcolor{cyan}{[CoT]}: The CoT generated by the criticizer.


\end{itemize}
\end{custombox}

\begin{custombox}{[Image Classification] Annotation Prompt - naïve}
\textbf{Prompt} 
\\
\textcolor{purple}{\{image\_data\}} 
\\
Determine the label of the image classification task. The list of labels is: \textcolor{purple}{\{label\_list\_with\_index\}}. The required output format is: [label\_index]. For example, if the label is \textcolor{purple}{\{first\_label\}}, you should output [0]. Do not return other texts. 
\\
\textbf{Output}
\\
\textcolor{cyan}{[label\_index]}
\end{custombox}


\begin{custombox}{[Text Classification] Annotation Prompt - naïve}
\textbf{Prompt} 
\\
Determine the label of the text classification task. The text is \textcolor{purple}{\{text\_data\}}. The list of labels is: \textcolor{purple}{\{label\_list\_with\_index\}}. The required output format is: [label\_index]. For example, if the label is \textcolor{purple}{\{first\_label\}}, you should output [0]. Do not return other texts. 
\\
\textbf{Output}
\\
\textcolor{cyan}{[label\_index]}
\end{custombox}

\begin{custombox}{[VQA-Binary] Annotation Prompt - naïve}
\textbf{Prompt} 
\\
\textcolor{purple}{\{image\_data\}} 
\\
Answer the question based on the given image. The question is: \textcolor{purple}{\{question\}}. The required output format is [0] for No and [1] for Yes. Do not return other text.  
\\
\textbf{Output}
\\
\textcolor{cyan}{[answer\_index]}
\end{custombox}


\begin{custombox}{[Image Classification] Annotation Prompt - CoT}
\textbf{Prompt} 
\\
\textcolor{purple}{\{image\_data\}} 
\\
Determine the label of the image classification task. The list of labels is: \textcolor{purple}{\{label\_list\_with\_index\}}. The required output format is: [label\_index]. Think step-by-step and provide your reasoning. Example of required output format is: [reasoning][label\_index]. The first brackets contain your step-by-step reasoning, and the second brackets contain the label index such as [0] for \textcolor{purple}{\{first\_label\}}. Do not return other texts. 
\\
\textbf{Output}
\\
\textcolor{cyan}{[CoT\_A][label\_index]}
\end{custombox}

\clearpage

\begin{custombox}{[Image Classification] Black-box Criticism Prompt - naïve}
\textbf{Prompt} 
\\
\textcolor{purple}{\{image\_data\}} 
\\
Your task is to produce the probability that the label of the given image is wrong. The list of labels is: \textcolor{purple}{\{label\_list\_with\_index\}}. The label of the image is:  \textcolor{purple}{\{label\_index\}}. The required output format is: [error\_probability]. For example, [0.911].\ The error probability should be reported in 3 decimals. Do not return other texts. 
\\
\textbf{Output}
\\
\textcolor{cyan}{[error\_probability]}
\end{custombox}


\begin{custombox}{[Image Classification] Black-box Criticism Prompt - CoT}
\textbf{Prompt} 
\\
\textcolor{purple}{\{image\_data\}} 
\\
Your task is to produce the probability that the label of the given image is wrong. The list of labels is: \textcolor{purple}{\{label\_list\_with\_index\}}. The label of the image is:  \textcolor{purple}{\{label\_index\}}. Think step-by-step and provide your reasoning. The required output format is: [reasoning][error\_probability]. The first brackets contain your step-by-step reasoning, and the second brackets contain the error probability such as [0.911]. The error probability should be reported in 3 decimals. Do not return other texts.
\\
\textbf{Output}
\\
\textcolor{cyan}{[CoT][error\_probability]}
\end{custombox}


\begin{custombox}{[Image Classification] Black-box Criticism Prompt - multiple choice}
\textbf{Prompt} 
\\
\textcolor{purple}{\{image\_data\}} 
\\
Your task is to analyze if label of the given image is wrong and select from [1: correct, 2: correct but not sure, 3: not sure, 4: incorrect but not sure, 5: incorrect]. The list of labels is: \textcolor{purple}{\{label\_list\_with\_index\}}. The label of the image is:  \textcolor{purple}{\{label\_index\}}. Think step-by-step and provide your reasoning. The required output format is: [reasoning][error\_level]. The first brackets contain your step-by-step reasoning, and the second brackets contain the error level such as [5] for incorrect. Do not return other texts.
\\
\textbf{Output}
\\
\textcolor{cyan}{[CoT][error\_level]}
\end{custombox}


\begin{custombox}{[Image Classification] Black-box Criticism Prompt - devil's advocate}
\textbf{Prompt} 
\\
\textcolor{purple}{\{image\_data\}} 
\\
Your task is to produce the probability that the statement related to the label of the given image is wrong. The list of labels is: \textcolor{purple}{\{label\_list\_with\_index\}}. The statement of the image label is:  \textcolor{purple}{[CoT\_A]}. Think step-by-step and provide your reasoning. The required output format is: [reasoning][error\_probability]. The first brackets contain your step-by-step reasoning, and the second brackets contain the error probability such as [0.911]. The error probability should be reported in 3 decimals. Do not return other texts.
\\
\textbf{Output}
\\
\textcolor{cyan}{[CoT][error\_probability]}
\end{custombox}

\clearpage


\begin{custombox}{[Image Classification] White-box Criticism Prompt - naïve}
\textbf{Prompt} 
\\
\textcolor{purple}{\{image\_data\}} 
\\
Your task is to decide whether the label of the given image is wrong. The list of labels is: \textcolor{purple}{\{label\_list\_with\_index\}}. The label of the image is:  \textcolor{purple}{\{label\_index\}}. The required output is either Yes or No, where Yes means mistake and No otherwise. Do not return other texts. 
\\
\textbf{Output}
\\
\textcolor{cyan}{Yes/No}
\end{custombox}



\begin{custombox}{[Image Classification] White-box Criticism Prompt - CoT}
\textbf{Prompt} 
\\
\textcolor{purple}{\{image\_data\}} 
\\
Your task is to decide whether the label of the given image is wrong. The list of labels is: \textcolor{purple}{\{label\_list\_with\_index\}}. The label of the image is:  \textcolor{purple}{\{label\_index\}}. Think step-by-step and provide your reasoning. The required output format is: [reasoning][answer]. The first brackets contain your step-by-step reasoning, and the second brackets contain either Yes or No with Yes meaning mistake and No otherwise. Do not return other texts. 
\\
\textbf{Output}
\\
\textcolor{cyan}{[CoT][Yes/No]}
\end{custombox}










==> Figures/appendices/apx4-proofs.tex <==
\section{\textbf{Theoretical Proofs}} \label{apx: proofs}

\subsection{Proof of Proposition 5.1 - Statistical Properties of ACT Loss (Variance)}

\begin{proof}
Recall that the ACT loss is defined as:
\begin{equation}\label{eq:apx_act_loss}
\mathcal{L}^{(\mathrm{ACT})}_\btheta = \frac{1}{N} \sum_{i = 1}^N \left(  
 \ell^{(m)}_{\btheta, i} + \left(\ell_{\btheta, i} - \ell^{(m)}_{\btheta, i}\right) \frac{\delta_i(B)}{\pi_B(\hat{\epsilon}_i)} \right),
\end{equation}
where $\delta_i(B) \sim \mathbb{B}(\pi_B(\hat{\epsilon}_i))$. Then, we define
\[
Z_i := \ell^{(m)}_{\btheta, i} + \left(\ell_{\btheta, i} - \ell^{(m)}_{\btheta, i}\right) \cdot \frac{\delta_i(B)}{\pi_B(\hat{\epsilon}_i)},
\quad \text{and} \quad
Z := \frac{1}{N} \sum_{i=1}^N Z_i = \mathcal{L}_\btheta^{(\mathrm{ACT})}.
\]

Assuming that data are i.i.d, the variance of the ACT loss is now equivalent to the variance of $Z$, which is
\begin{align}
\operatorname{Var}(Z) &= \operatorname{Var}\left( \frac{1}{N} \sum_{i=1}^N Z_i \right) 
= \frac{1}{N^2} \sum_{i=1}^N \operatorname{Var}(Z_i).
\end{align}

Hence, it suffices to only calculate the variance of $Z_i$, which can be decomposed into two parts as $\operatorname{Var}(Z_i) = \mathbb{E}[Z_i^2] - (\mathbb{E}[Z_i])^2$. We first expand:
\begin{align}
Z_i^2 &= \left( \ell^{(m)}_{\btheta,i} + \left(\ell_{\btheta,i} - \ell^{(m)}_{\btheta,i} \right) \cdot \frac{\delta_i(B)}{\pi_B(\hat{\epsilon}_i)} \right)^2 \notag \\
&= \left( \ell^{(m)}_{\btheta,i} \right)^2 
+ 2 \ell^{(m)}_{\btheta,i} (\ell_{\btheta,i} - \ell^{(m)}_{\btheta,i}) \cdot \frac{\delta_i(B)}{\pi_B(\hat{\epsilon}_i)} 
+ (\ell_{\btheta,i} - \ell^{(m)}_{\btheta,i})^2 \cdot \frac{\delta_i(B)}{\pi_B(\hat{\epsilon}_i)^2},
\end{align}
where we have $\delta^2_i(B) = \delta_i(B)$ because $\delta_i(B)$ is either $0$ or $1$. We assume that $\delta_i(B)$ and $\ell_{\btheta,i}$ are independent. In addition, it is easy to see that $\mathbb{E}[\delta_i(B)] = \pi_B(\hat{\epsilon}_i)$, and that $\mathbb{E}[Z_i] = \mathbb{E}[\ell_{\btheta,i}]$. So, we calculate the expectation of $Z_i^2$ as follows:
\begin{align}
\mathbb{E}[Z_i^2] &=  \left( \ell^{(m)}_{\btheta,i} \right)^2 + 2 \ell^{(m)}_{\btheta,i} \mathbb{E}\left[\ell_{\btheta,i} - \ell^{(m)}_{\btheta,i}\right] +\mathbb{E} \left[\left(\ell_{\btheta,i} - \ell^{(m)}_{\btheta,i}\right)^2 \cdot  \frac{1}{\pi_B(\hat{\epsilon}_i)}\right] \notag\\
&= \mathbb{E}\left[\ell_{\btheta,i}^2 - \left(\ell_{\btheta,i} - \ell^{(m)}_{\btheta,i}\right)^2  \right] + \mathbb{E} \left[\left(\ell_{\btheta,i} - \ell^{(m)}_{\btheta,i}\right)^2 \cdot  \frac{1}{\pi_B(\hat{\epsilon}_i)}\right] \notag\\
&= \mathbb{E}\left[\ell_{\btheta,i}^2\right] + \mathbb{E} \left[\left(\ell_{\btheta,i} - \ell^{(m)}_{\btheta,i}\right)^2 \cdot  \left(\frac{1}{\pi_B(\hat{\epsilon}_i)} - 1 \right)\right]
\end{align}

Thus, we have 
\begin{align}
    \operatorname{Var}(Z_i) &= \mathbb{E}\left[\ell_{\btheta,i}^2\right] + \mathbb{E} \left[\left(\ell_{\btheta,i} - \ell^{(m)}_{\btheta,i}\right)^2 \cdot  \left(\frac{1}{\pi_B(\hat{\epsilon}_i)} - 1 \right)\right] - \mathbb{E}^2[\ell_{\btheta,i}]\notag\\
    &= \operatorname{Var}(\ell_{\btheta,i}) + \mathbb{E} \left[\left(\ell_{\btheta,i} - \ell^{(m)}_{\btheta,i}\right)^2 \cdot  \left(\frac{1}{\pi_B(\hat{\epsilon}_i)} - 1 \right)\right]
\end{align}


Finally, we can show that
\begin{align}
\operatorname{Var}\left(\mathcal{L}^{(ACT)}\right) = \operatorname{Var}(Z) &= \frac{1}{N^2} \sum_{i=1}^N \operatorname{Var}(Z_i)  \notag\\
&= \frac{1}{N^2} \sum_{i=1}^N \left( \operatorname{Var}(\ell_{\btheta,i}) + \mathbb{E} \left[\left(\ell_{\btheta,i} - \ell^{(m)}_{\btheta,i}\right)^2 \cdot  \left(\frac{1}{\pi_B(\hat{\epsilon}_i)} - 1 \right)\right] \right) \notag \\
&= \frac{1}{N} \left( \operatorname{Var}(\ell_\btheta) + \mathbb{E}\left[ \left( \ell_\btheta - \ell^{(m)}_\btheta \right)^2 \cdot \left( \frac{1}{\pi_B(\hat{\epsilon})} - 1 \right) \right] \right).
\end{align}
This completes the proof.
\end{proof}




\clearpage

\subsection{Proof of Theorem 5.2 - Probabilistic Upper Bound of the Parameter Gap} 

\begin{proof}
From the definition of ACT loss in Equation \eqref{eq:apx_act_loss}, we can show that
\begin{align}
    \nabla \mathcal{L}_\theta^{(ACT)} &= \frac{1}{N} \sum_{i=1}^N \pi_i \nabla \ell_{\theta,i}  + \frac{1}{N} \sum_{i=1}^N (1- \pi_i) \nabla \ell_{\theta,i}^{(m)} \notag \\
    &= \nabla \mathcal{L}_\theta + \big( \frac{1}{N}\sum_{i=1}^N \pi_i \nabla \ell_{\theta,i}  - \frac{1}{N}\sum_{i=1}^N  \nabla \ell_{\theta,i} \big) + \frac{1}{N} \sum_{i=1}^N (1- \pi_i)  \nabla \ell_{\theta,i}^{(m)} \notag \\
    &= \nabla \mathcal{L}_\theta + \frac{1}{N} \sum_{i=1}^N (1 - \pi_i) \left( \nabla \ell_{\theta,i}^{(m)} - \nabla \ell_{\theta,i}  \right)
\end{align}
where we let $\pi_i  = \frac{\delta_i(B)}{\pi_B(\hat \epsilon_i)} $ and $\mathcal{L}_\theta = \frac{1}{N}\ell_{\btheta,i}$. 

It is easy to see $\mathbb{E} \left[(1- \pi_i) \left( \nabla \ell_{\theta,i}^{(m)} - \nabla \ell_{\theta,i} \right) \right] = 0$.  Assume there exist constants $q, C > 0$ such that the transformed error $\pi_B(\hat \epsilon_i) \geq q \ $ for all $i$ with $\delta_i(B) = 1$, and the gradient gap $\left\|\nabla \ell_{\theta,i}^{(m)} - \nabla \ell_{\theta,i}\right\| \leq C$ for all $i \in \{1, 2, ..., N\}$.  Next, we bound for any $i$ that 
\begin{align*}
    &\left\| (1- \pi_i) \left( \nabla \ell_{\theta,i}^{(m)} - \nabla \ell_{\theta,i} \right) \right\| \leq \left|1-\pi_i\right| \left\| \nabla \ell_{\theta,i}^{(m)} - \nabla \ell_{\theta,i} \right\| \leq \max\left\{1, \frac{1-q}{q} \right\} C =: c_0, \\
    &\text{and} \quad \mathbb E \left\|  (1- \pi_i) \left( \nabla \ell_{\theta,i}^{(m)} - \nabla \ell_{\theta,i} \right) \right\|^2  \leq \mathbb{E} \left[(1-\pi_i)^2\right] \left\| \nabla \ell_{\theta,i}^{(m)} - \nabla \ell_{\theta,i} \right\|^2 \leq \frac{1-q}{q} C^2 =: c_1.
\end{align*}
Then we apply the vector Bernstein's inequality (e.g., Lemma 18 in \cite{kohler2017sub}) such that
\begin{align}
    \mathbb P \left( \left\| \frac{1}{N} \sum_{i=1}^N (1 - \pi_i) \left( \nabla \ell_{\theta,i}^{(m)} - \nabla \ell_{\theta,i} \right) \right\| \geq \epsilon \right) \leq 2\exp\left( -N \epsilon^2/(8 c_1) \right) 
\end{align}
for $0< \epsilon < \frac{c_1}{c_0}$. Then, with a probability of at least $1- p$ where $p \in (0,1)$, we have 
\begin{align}
    \left\| \frac{1}{N}\sum_{i=1}^N (1 - \pi_i) \left( \nabla \ell_{\theta,i}^{(m)} - \nabla \ell_{\theta,i} \right) \right\| \leq \sqrt{\frac{ 8 c_1 \log(2/p)}{N}}
\end{align}
for any $N \geq 8c_0^2 \log(2/p)/c_1$. 

Finally, due to the $\mu$-strong convexity of $\ell_{\theta,i}^{(\cdot)}$ and thus $\mathcal{L}_\theta^{(\cdot)}$, with a probability of at least $1-p$, we can bound the parameter gap
\begin{align}
    \left\| \theta^{(ACT)}_* - \theta_* \right\| &\leq \frac{1}{\mu} \left\| \nabla \mathcal{L}_{\theta_*^{(ACT)}}^{(ACT)} - \nabla \mathcal{L}_{\theta_*}^{(ACT)} \right\| \notag\\
    &= \frac{1}{\mu} \left\|    \nabla \mathcal{L}_{\theta_*} - \nabla \mathcal{L}_{\theta_*}^{(ACT)}   \right\| \notag\\
    &= \frac{1}{\mu} \left\| \frac{1}{N} \sum_{i=1}^N (1 - \pi_i) \left( \nabla \ell_{\theta_*,i}^{(m)} - \nabla \ell_{\theta_*,i}  \right) \right\| \notag\\
    &\leq \sqrt{\frac{8c_1 \log(2/p)}{\mu^2 N}}
\end{align}
where $\theta^{(ACT)}_* = \arg\min_\theta \mathcal{L}_\theta^{(ACT)}$, and $\theta_* = \arg\min_\theta \mathcal{L}_\theta$.

This completes the proof.
\end{proof}


==> Figures/appendices/apx5-losses.tex <==
\section{\textbf{Further Details of ACT Losses}}\label{apx: losses}

\subsection{ACT Losses with Different Sampling Rules}

The ACT losses with different sampling rules are listed as follows:

\begin{itemize}
    \item \textit{Normalization} \citep{gligoric2024can,zrnic2024active}
    \begin{equation}
    \mathcal{L}^{(\mathrm{ACT})}_\btheta = \frac{1}{N} \sum_{i = 1}^N \left(  
     \lambda \ell^{(m)}_{\btheta, i} + \left(\ell_{\btheta, i} - \lambda \ell^{(m)}_{\btheta, i}\right) \times \frac{\delta_i(B) \times \sum_{n=1}^N \hat{\epsilon}_n}{B \times \hat{\epsilon}_i} \right);
    \end{equation}
    

    \item \textit{Exponential Weighting}
    \begin{equation}
    \mathcal{L}^{(\mathrm{ACT})}_\btheta = \frac{1}{N} \sum_{i = 1}^N \left(  
     \lambda \ell^{(m)}_{\btheta, i} + \left(\ell_{\btheta, i} - \lambda \ell^{(m)}_{\btheta, i}\right) \times \delta_i(B) \left(1+\mathrm{e}^{-\beta(\hat{\epsilon}_i - \alpha)}\right) \right);
    \end{equation}

    \item \textit{Thresholding}
    \begin{equation}
    \mathcal{L}^{(\mathrm{ACT})}_\btheta = \frac{1}{N} \sum_{i = 1}^N \left(  
     \lambda \ell^{(m)}_{\btheta, i} + \left(\ell_{\btheta, i} - \lambda \ell^{(m)}_{\btheta, i}\right) \times \delta_i(B)\right),
    \end{equation}
    
\end{itemize}

where $\lambda \in [0,1]$ is the power tuning parameter \citep{gligoric2024can,angelopoulos2023ppi++}, which controls the extent to which machine annotations are utilized. Specifically, $\lambda = 0$ corresponds to completely ignoring machine annotations, while $\lambda = 1$ corresponds to the full usage. Notably, when employing the thresholding sampling rule with $\lambda = 1$, the ACT loss is equivalent to the standard Cross-entropy loss computed using human-annotated labels when available, and machine-annotated labels otherwise. Therefore, we stated in Section 5.2 that the Cross-entropy loss is a special case of the ACT loss.




\subsection{Distributions of Transformed Errors with Different Sampling Rules}

In Figure \ref{fig: apx_loss_error}, we present the distributions of transformed errors for data samples reviewed by humans ($\delta(B) = 1$) under different sampling strategies. We observe that, with normalization sampling, the lower bounds of the transformed errors are close to 0 across all presented datasets. In contrast, for exponential weighting, the lower bounds typically around 0.8, while thresholding yields a consistent lower bound of 1.0. Based on Theorem 5.2, these results provide an explanation for why exponential weighting and thresholding can lead to better downstream training performance.

\vspace{-1cm}

\begin{figure} [b]
    \centering
    \includegraphics[width=1\linewidth]{Figures/apx_loss_error.pdf}
    \caption{Distributions of transformed errors with different sampling rules ($\delta(B) = 1$). $B$ is set to the ideal human budget for each dataset.}
    \label{fig: apx_loss_error}
\end{figure}

==> Figures/appendices/apx6-sensitivity_human_budget.tex <==
\section{\textbf{Sensitivity Analyses of Human Budget}} \label{apx: sens_human}

\subsection{AQG vs. Human Budget}
In Figure \ref{fig: apx_sens_aqg}, we illustrate how Annotation Quality Gain (AQG) changes with the human budget proportion. We observe that as the human budget increases, AQG generally rises rapidly at first, then begins to plateau after a certain point. This initial rapid increase suggests that the human-corrected samples tend to be more obvious and easily identifiable errors. On most datasets, AQG does not reach 100\% before the human budget reaches its maximum. In other words, it is usually difficult to achieve perfect annotation quality without reviewing all examples. This indicates that some subtle or hard-to-detect errors are unavoidable. However, we will show in Figure \ref{fig: apx_sens_downstream} that this does not undermine the effectiveness of using ACT to reduce human effort. With the ACT loss, a promising downstream training does not rely on perfectly labeled data.



\begin{figure}[h!]
    \centering
    \includegraphics[width=1\linewidth]{Figures/apx_sens_aqg.pdf}
    \caption{How AQG changes with human budget (\%). The results are presented for GPT4o self-criticism with 4 black-box strategies.}
    \label{fig: apx_sens_aqg}
\end{figure}




\clearpage
\subsection{Downstream Performance vs. Human Budget}
We conducted the human budget sensitivity experiments using GPT4o self-criticism and the thresholding sampling rule. The results are shown in Figure \ref{fig: apx_sens_downstream}. We observe that both annotation accuracy and downstream accuracy generally increase with a larger human budget. When using the ideal budget, a performance gap can be observed across all datasets. This is because the criticizer is not perfectly accurate, leading to some overlooked mislabeled data, which slightly degrades the final training performance. In Figure \ref{fig: apx_sens_downstream}, we also show the downstream performance gain achieved by adding a 10\% buffer budget on top of the ideal budget. In 4 out of 6 datasets, this buffer nearly eliminates the performance gap, while the gap is significantly reduced in the other 2 datasets. \textbf{Therefore, we recommend first evaluating the annotator's accuracy, and then adding a reasonable buffer to the ideal budget based on the observed error rate.}

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{Figures/apx_sens_downstream.pdf}
    \caption{How annotation accuracy and downstream accuracy change with the human budget (\%). The black vertical line shows the position of the ideal human budget (i.e., one minus the initial annotator accuracy). The grey area shows the buffer budget over the ideal budget.}
    \label{fig: apx_sens_downstream}
\end{figure}

==> Figures/appendices/apx7-related_works___comparison.tex <==
\section{\textbf{Extended Discussions and Experiments}} \label{apx: related_works}

\subsection{Additional Related Works}
\textbf{Enhance Data Annotation with LLMs}

To improve the quality of LLM annotation, AdaICL adopts in-context learning (ICL) with examples annotated by human \citep{mavromatis2023examples}. The ICL examples are actively selected based on LLM logit probabilities during annotation, which means their method only supports white-box LLMs. In addition, AdaICL lacks mechanisms for long-context visual inference, making it difficult to apply directly to vision-based tasks. This is because retrieving and encoding a large number of visual examples during inference would incur prohibitive computational costs \citep{wan2024lookm, wang2024longllava}. However, we consider ICL as a potential direction for future work, particularly as a component in our data pipeline for building an annotator. 

Other related works typically follow a three-step LLM-human collaborative framework: (1) LLMs generate initial labels, (2) a verifier assesses the correctness of these labels and outputs verification scores, and (3) human annotators re-annotate a selected subset of labels based on these scores \citep{kim2024meganno+, wang2024human_llm, gligoric2024can, wang2024model}. The primary distinction among these methods lies in the design of the verifier. For instance, Model-in-the-Loop (MILO) \citep{wang2024model} utilizes the logit scores from another LLM-based verifier (similar to our white-box criticizer). In contrast, MEGAnno+ \citep{kim2024meganno+} directly employs the logit probabilities from the LLM annotator itself. Another framework proposed by \citep{wang_model---loop_2024} uses a verifier implemented as a Support Vector Machine \citep{cortes1995support}, Random Forests \citep{breiman2001random}, or BERT \citep{devlin2018bert}, trained on additional human-annotated data. Unlike our approach, the aforementioned methods focus solely on annotation accuracy without considering the utility of annotations for downstream training. This narrow focus limits their effectiveness, as high-accuracy labels do not necessarily translate into meaningful model improvements.


% Another study introduced Model-in-the-Loop (MILO), a collaborative annotation system combining LLMs and human experts to enhance the efficiency and quality of multimodal data annotation \citep{wang2024model}. While the paper demonstrates improvements in time and data quality, it does not delve into strategies for optimizing the MILO data pipeline through model selection or prompt engineering. Additionally, different from our work, it does not explore methods for leveraging the annotated data to improve downstream training outcomes.


% Wang et al. \citep{wang2024human_llm} also proposed a human-LLM collaborative data annotation framework. The framework consists of three stages: (1) LLMs generate labels and explanations, (2) a verifier evaluates the quality of the LLM-generated labels, and (3) human annotators re-annotate a subset of labels that receive lower verification scores. Unlike our ACT data pipeline, the verifier, which is functionally similar to the criticizer, is implemented using a trained Support Vector Machine \citep{cortes1995support}, Random Forests \citep{breiman2001random}, or BERT \citep{devlin2018bert}, and trained with additional human-annotated data.

% MEGAnno+ \citep{kim2024meganno+} is also a human-LLM collaborative data pipeline, 

The most relevant work to our research is CDI \citep{gligoric2024can}, which identifies LLM errors using a trained XGBoost model \citep{chen2016xgboost} and relies on human annotators for correction. During the annotation process, CDI prompts annotators to provide both labels and corresponding verbalized confidence scores. These confidence scores are provided in a black-box manner, where higher values indicate greater confidence. For example, an annotator might respond, “The label is cat, and my confidence is 0.999,” to express high certainty. The XGBoost model then uses these confidence scores as input to learn and predict error probabilities. The ground truth is either 0 or 1 depending on the correctness of the annotation, and then the logit probabilities are regarded as error probabilities. However, CDI has two key limitations: (1) its error detection mechanism lacks flexibility, requiring task-specific design and additional training data, and (2) it employs a normalization-based active M-estimation loss, which we find suboptimal in downstream tasks.

% In the following experimental comparison, we primarily focus on the CDI approach for several reasons. First, AdaICL lacks mechanisms for long-context visual inference, making it difficult to apply directly to vision-based tasks. This is because retrieving and encoding a large number of visual examples during inference would incur prohibitive computational costs \citep{wan2024lookm, wang2024longllava}. However, we consider ICL as a potential direction for future work, particularly as a component in our data pipeline for building an annotator. Second, MILO does not provide a deployable data pipeline, which limits its utility for practical evaluation. Third, the human-LLM framework proposed in \citep{wang2024human_llm} trains the verifier using only text-based features, making it similarly challenging to adapt for vision tasks. However, we note that this method is conceptually aligned with CDI in that it also introduces a separately trained model to serve as a criticizer or verifier. Therefore, in the following analysis, we will compare two approaches for generating criticism: one based on a trained model (e.g., CDI with XGBoost), and the other leveraging a pre-trained LLM without additional training.

\clearpage

\subsection{Potential Improvements of ACT}
Here, we outline several potential improvements to the ACT data pipeline, as inspired by the related works. First, drawing from AdaICL \citep{mavromatis2023examples}, we could enhance the prompts of the MLLM annotator—particularly for NLP tasks—by incorporating in-context examples. Second, following the approach of MEGAanno+ \citep{kim2024meganno+}, it may be beneficial to combine the annotator's confidence scores with the criticizer's error estimations to better capture the insights from both perspectives. Finally, while the current pipeline relies on a single MLLM annotator–criticizer pair, it could be extended to a multi-model setup using techniques such as majority voting or peer discussion in \citep{tseng2024expert}. An illustration is provided in Figure \ref{fig: apx_improvement}.

For decision of the human budget, one may consider dynamically estimating and adjusting the human budget during the review process. As more human-verified labels are accumulated over time, it becomes increasingly feasible to refine the error rate estimation and update the budget allocation accordingly.

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{Figures/apx_improvement.pdf}
    \caption{Illustration of potential improvements of the ACT data pipeline.}
    \label{fig: apx_improvement}
\end{figure}





\subsection{Supplementary Experiments}

\subsubsection{Comparison with CDI}

In Table \ref{tab: cdi_downstream}, we compare the downstream performance of models trained on ACT and CDI data using various loss functions. Note that CDI data with the ACT norm. loss is corresponding to the approach proposed in \citep{gligoric2024can}. We apply the same human budget (the ideal human budget) to both ACT and CDI. For CDI, a proportion of this budget is allocated to training the XGBoost error detector. The results demonstrate that ACT consistently outperforms CDI in reducing the downstream performance gap.

\begin{table}[h]
\caption{Comparison between ACT and CDI in downstream tasks. The test accuracy (\%) is reported in form of mean $\pm$ std over 5 runs.
}\label{tab: cdi_downstream}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|llllll}
\toprule
Training Data -   Loss              & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}CIFAR10\\ (ResNet18)\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Fashion\\ (ResNet18)\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Cars\\ (ResNet18)\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Emotion\\ (RoBERTa)\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Irony\\ (RoBERTa)\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}VQA-RAD\\ (BLIP-VQA)\end{tabular}}\\ \midrule
Human only - Cross-entropy Loss     & 88.66 $\pm$ 0.97                                                    & 93.01 $\pm$ 0.63                                                    & 87.88 $\pm$ 0.36  & 81.82 $\pm$ 0.57 &  70.18 $\pm$ 3.23                                             & 67.81 $\pm$ 1.47                                                    \\ \midrule
CDI data - Cross-entropy loss 
&     84.02 $\pm$ 0.85                                         &     86.99 $\pm$ 0.72                                 
&    85.61 $\pm$  0.24     
& 79.91 $\pm$ 1.37 
&  66.63 $\pm$ 3.44                        
&    61.77 $\pm$  3.41                                        \\

CDI data - ACT norm. loss
&    72.22 $\pm$  1.71                                        &     83.38 $\pm$ 1.79                               
&    10.76 $\pm$ 1.12  
&  79.05 $\pm$ 1.15
&    65.96 $\pm$ 3.36                            
&    62.24 $\pm$  3.05                                         \\

CDI data - ACT exp. loss 
&    84.99 $\pm$ 0.31                                       &        87.72 $\pm$  0.54                          
&   86.03  $\pm$  0.15     
&  80.51 $\pm$ 1.49
&   68.44 $\pm$  2.22                          
&   67.33  $\pm$  1.66                                         \\
CDI data - ACT thre. loss
&     84.91 $\pm$  0.57                                        &  87.64 $\pm$ 0.52                        
&   85.89 $\pm$ 0.27     
&  80.00 $\pm$ 0.83
&    68.19 $\pm$ 2.29                           
&   67.44  $\pm$ 2.16                                     \\ \midrule

ACT data - Cross-entropy loss           &  85.59 $\pm$ 0.52                                                     &  87.50 $\pm$ 0.86                                                   &  85.88 $\pm$ 0.26            & 80.82 $\pm$ 1.08 & 67.83 $\pm$ 2.82                                       &  61.83 $\pm$ 3.27                                                    \\ 
ACT data - ACT norm. loss           & 64.70 $\pm$ 5.46                                                     & 69.27 $\pm$ 7.25                                                    & 11.54 $\pm$ 0.96     & 79.87 $\pm$ 0.88 & 65.66 $\pm$ 2.00                                               & 62.55 $\pm$ 3.01                                                    \\ 
\textbf{ACT data - ACT exp. loss (Ours)}   & 87.73 $\pm$ 0.36                                                    & 89.73 $\pm$ 0.35                                                    & 86.19 $\pm$ 0.14    & 81.44 $\pm$ 0.51 & 68.49 $\pm$ 3.20                                              & 67.73 $\pm$ 1.33                                                    \\
\textbf{ACT data - ACT thre. loss (Ours)}  & 87.95 $\pm$ 0.35                                                    & 89.16 $\pm$ 0.89                                                    & 86.00 $\pm$ 0.26     & 81.41 $\pm$ 0.64 & 68.21 $\pm$  1.94                                             & 67.02 $\pm$ 1.32                                                    \\ \midrule
Human-CDI performance gap (\%)               
& \multicolumn{1}{c}{ 3.67\%}                     & \multicolumn{1}{c}{ 5.29\%}                    & \multicolumn{1}{c}{ 1.85\%}                     & \multicolumn{1}{c}{ 1.31\%}
& \multicolumn{1}{c}{ 1.74\%}
& \multicolumn{1}{c}{ 0.37\%} \\ 
\rowcolor[HTML]{EFEFEF} 
Human-ACT performance gap (\%)               
& \multicolumn{1}{c}{0.71\%}                                                      
& \multicolumn{1}{c}{3.28\%}                                                      
& \multicolumn{1}{c}{1.69\%}                  
& \multicolumn{1}{c}{0.38\%}
& \multicolumn{1}{c}{1.69\%}                     & \multicolumn{1}{c}{0.08\%} \\ 
Human budget (\%)               & \multicolumn{1}{c}{11.52\%}                                                      & \multicolumn{1}{c}{21.81\%}                                                      & \multicolumn{1}{c}{9.56\%}                     & \multicolumn{1}{c}{17.98\%}
& \multicolumn{1}{c}{33.79\%}                               & \multicolumn{1}{c}{30.15\%} \\ 
\bottomrule
\end{tabular}}
\end{table}

\clearpage

\subsubsection{Comparison with Active Learning and Pseudo Labels}

We compare our method with more existing baselines from related fields on CIFAR10 (ResNet18):

\begin{itemize}
    \item \textbf{Pseudo Labelling}: We randomly label 11.52\% of the data to fine-tune ResNet18, then iteratively add high-confidence predictions (e.g., logit probability > 0.9) as pseudo labels to the training set.

    \item \textbf{Active Pseudo Labelling}: We start by labelling 100 samples per class and progressively select uncertain samples (based on prediction entropy) for annotation until the human budget is exhausted.
    
\end{itemize}

The results shown in Table \ref{tab:apx_pseudo_active} indicate that our approach outperforms these two methods by 4.28\% and 2.56\% in terms of performance gap from 100\% human annotation.


\begin{table}[ht]
\centering
\caption{Comparison with baselines from related fields.}
\label{tab:apx_pseudo_active}
\rowcolors{2}{gray!10}{white}
\renewcommand{\arraystretch}{1.5}
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{l|cc}
\toprule
\textbf{Method} & \textbf{Accuracy (\%)} & \textbf{Human Performance Gap (\%)} \\
\midrule
Human-only -- CE loss             & $88.66 \pm 0.97$ & --   \\
\midrule
ACT -- ACT thre. loss (Ours)             & $87.95 \pm 0.35$ & 0.71 \\ 
Pseudo labeling -- CE loss        & $83.67 \pm 0.32$ & 4.99 \\
Active Pseudo labeling -- CE loss & $85.39 \pm 0.91$ & 3.27 \\
\bottomrule
\end{tabular}}
\end{table}

\subsubsection{More Challenging Tasks: Biased and Long-tail Data}

To validate the effectiveness of our method in more challenging tasks, we conduct two experiments:

\begin{itemize}
    \item Allenoise \citep{rkaczkowska2024allenoise} is a product classification dataset where similar category names often result in subjective and biased labelling. We focus on 20 labels under the "Sports \& Travel" category, which exhibit approximately 70\% label similarity—making the task ambiguous and prone to bias. Additionally, the largest category contains 27 times more samples than the smallest, reflecting a significant long-tail distribution. The results are shown in Table \ref{tab:apx_allenoise_roberta}, demonstrating that ACT yields only a 1.4\% performance gap in accuracy and a 0.0041 difference in F1-score compared to full human annotation.
    \begin{table}[ht]
\centering
\caption{Experiment results on AlleNoise with RoBERTa.}
\label{tab:apx_allenoise_roberta}
\rowcolors{2}{gray!10}{white}
\renewcommand{\arraystretch}{1.5}
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{l|cc}
\toprule
\textbf{Data -- Loss (AlleNoise -- RoBERTa)} & \textbf{Accuracy (\%)} & \textbf{F1-score} \\
\midrule
Human annotation -- CE loss                 & $91.54 \pm 1.84$ & $0.8448 \pm 0.0165$ \\
ACT data -- ACT thre. loss (GPT4o self-criticism) & $90.14 \pm 1.79$ & $0.8397 \pm 0.0191$ \\
\textbf{Human--ACT performance gap}         & 1.40 & 0.0041 \\
\bottomrule
\end{tabular}}
\end{table}


    \item CIFAR10-LT \footnote{\url{https://huggingface.co/datasets/tomas-gajarsky/cifar10-lt}} is a long-tailed variant of CIFAR10 with an imbalance ratio of 100 between the most and least frequent classes. As shown in Table \ref{tab:apx_cifar10lt_resnet}, ACT achieves a performance gap of 1.97\% in accuracy and 0.0148 in F1-score compared to full human annotation.

    \begin{table}[ht]
\centering
\caption{Experiment results on CIFAR10-LT with ResNet.}
\label{tab:apx_cifar10lt_resnet}
\rowcolors{2}{gray!10}{white}
\renewcommand{\arraystretch}{1.5}
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{lcc}
\toprule
\textbf{Data -- Loss (CIFAR10-LT -- ResNet)} & \textbf{Accuracy (\%)} & \textbf{F1-score} \\
\midrule
Human annotation -- CE loss                 & $70.29 \pm 2.15$ & $0.6820 \pm 0.0261$ \\
ACT data -- ACT thre. loss (GPT4o self-criticism) & $68.32 \pm 1.66$ & $0.6672 \pm 0.0263$ \\
\textbf{ACT -- Human performance gap}       & 1.97 & 0.0148 \\
\bottomrule
\end{tabular}}
\end{table}

\end{itemize}

\clearpage

\subsubsection{Analyses on Critic True Positives and False Positives
}

\textbf{a. Analyze Criticism Reliability with False Positives} 

Table \ref{tab:apx_fps} reports the number of false positives produced by different error detection methods across six datasets. The human budget is consistent with Table \ref{tab: downstream}. We compare GPT4o self-criticism and the best-performing cross-criticizer for each task, with random error sampling included as a baseline. We observe the following:

\begin{itemize}
    \item MLLM-based error detection significantly outperforms random sampling, consistently yielding fewer false positives across tasks.
    \item False positives account for approximately 5\%–15\% of the total dataset, depending on the complexity and ambiguity of the task.
\end{itemize}

These results suggest that MLLM-based criticism is an effective strategy for identifying annotation errors. In addition, there remains room for improvement, especially through incorporating sample-specific analysis and adaptive selection mechanisms in real-world applications.

\begin{table}[ht]
\centering
\caption{Number of false positives by different error detection methods across six datasets.}
\label{tab:apx_fps}
\rowcolors{2}{gray!10}{white}
\renewcommand{\arraystretch}{1.5}

% ---------- 第一行：前 3 个数据 ----------
\resizebox{\linewidth}{!}{
\begin{tabular}{l|ccc}
\toprule
\textbf{Error Detection Methods} & \textbf{CIFAR10 (data size$\sim$50k)} & \textbf{Fashion (data size$\sim$60k)} & \textbf{Cars (data size$\sim$8k)} \\
\midrule
Random Sampling        & 4866 & 9852 & 704 \\
GPT4o Self-Criticizer  & 2805 & 6395 & 594 \\
Optimal Cross-Criticizer & 2692 & 6087 & 514 \\
\bottomrule
\end{tabular}}

\vspace{0.5em} % 表格之间的间距

% ---------- 第二行：后 3 个数据 ----------
\resizebox{\linewidth}{!}{
\begin{tabular}{l|ccc}
\toprule
\textbf{Error Detection Methods} & \textbf{Emotion (data size$\sim$3k)} & \textbf{Irony (data size$\sim$3k)} & \textbf{VQA-RAD (data size$\sim$1k)} \\
\midrule
Random Sampling        & 480 & 640 & 198 \\
GPT4o Self-Criticizer  & 302 & 591 & 123 \\
Optimal Cross-Criticizer & 299 & 455 & 113 \\
\bottomrule
\end{tabular}}

\end{table}

\textbf{b. Compare Self- and Cross-Criticism with True Positives}

We use dataset VQA-RAD as an example, where GPT4o only achieves 69.85\% annotation accuracy. The human budget is set to 30.15\%. In Table \ref{tab:apx_tps}, we present the number of true positives and annotation accuracy after human correction. Randomly sampled errors are included as a baseline. It is clear that all MLLM criticizers perform much better than random sampling, while self- and cross-criticism do not show huge differences. This further strengthens the claim that self-criticism performs competitively with cross-criticism.

\begin{table}[ht]
\centering
\caption{Number of true positives and annotation accuracy after human correction (VQA-RAD).}
\label{tab:apx_tps}
\rowcolors{2}{gray!10}{white}
\renewcommand{\arraystretch}{1.5}
\resizebox{0.7\linewidth}{!}{
\begin{tabular}{l|cc}
\toprule
\textbf{Error Detection Methods} & \textbf{\#True Positives} & \textbf{Final Annotation Accuracy} \\
\midrule
Random Sampling    & 85  & 78.89\% \\
GPT4o (Self-criticism)       & 160 & 86.87\% \\
Gemini1.5P (Cross-criticism) & 153 & 86.12\% \\
Claude3.5S (Cross-criticism) & 159 & 86.76\% \\
LLaVA-OV (Cross-criticism)   & 158 & 86.66\% \\
Qwen2.5VL (Cross-criticism)  & 170 & 87.94\% \\
InternVL2.5 (Cross-criticism)& 149 & 85.70\% \\
\bottomrule
\end{tabular}}
\end{table}

\clearpage

\subsubsection{Ablation of Annotator-Criticizer Selection}

We conduct ablation experiments that examine how annotator-criticizer choice affects final downstream model performance. The experiments are conducted with Cars, because variations in self- and cross-criticism performance are large on this dataset based on Figure \ref{fig:exp_bx}. So, we would like to know whether the downstream performance also varies a lot.

In Table \ref{tab:apx_ablation}, we find that the effectiveness of criticism is indeed related to downstream performance. The best-performing criticizer (highest ABS) yields the smallest performance gap. However, the default GPT4o also performs reasonably well, keeping the gap within 2\%.

\begin{table}[ht]
\centering
\caption{Ablation on how annotator-criticizer choice affects final downstream model performance. The results are reported in ABS (\%) and accuracy (\%).}
\label{tab:apx_ablation}
\rowcolors{2}{gray!10}{white}
\renewcommand{\arraystretch}{1.5}
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccccc}
\toprule
\textbf{Cars -- GPT4o Annotation} & \textbf{GPT4o} & \textbf{Gemini1.5P} & \textbf{Claude3.5S} & \textbf{LLaVA-OV} & \textbf{Qwen2.5VL} & \textbf{InternVL2.5} \\
\midrule
Criticism ability -- ABS   & 60.6 & \textbf{70.9} & 53.2 & 55.9 & 54.4 & 57.5 \\
ACT data -- ACT thre. loss & $86.00 \pm 0.26$ & $\mathbf{86.21 \pm 0.31}$ & $85.21 \pm 0.35$ & $85.39 \pm 0.29$ & $85.80 \pm 0.29$ & $85.45 \pm 0.31$ \\
Human--ACT performance gap & 1.88 & \textbf{1.67} & 2.67 & 2.49 & 2.08 & 2.43 \\
\bottomrule
\end{tabular}}
\end{table}


\subsubsection{Cost-Benefit Analysis}

We present a cost-benefit analysis using CIFAR10 (50k samples) to compare three annotation strategies: (1) 100\% human annotation, (2) ACT with GPT4o self-criticism, and (3) ACT with GPT4o \& Qwen2.5VL cross-criticism. Note that we exclude the cases where GPUs are not rented but owned, whose costs are difficult to estimate. 

As shown in Table \ref{tab:apx_costs}, API-based approaches are the most cost-efficient. We also highlight that monetary costs are not the only concern. Human annotation also incurs significant time and educational costs, further highlighting the efficiency of our machine-based approach.

\begin{table}[ht]
\centering
\caption{Cost comparison between human-only annotation and ACT approaches.}
\label{tab:apx_costs}
\rowcolors{2}{gray!10}{white}
\renewcommand{\arraystretch}{1.6}
\scalebox{0.77}{
\begin{tabular}{p{5cm}|p{2.5cm}|p{5cm}|p{4cm}}
\toprule
\textbf{Item} & \textbf{Human-only} & \textbf{ACT (GPT4o-GPT4o)} & \textbf{ACT (GPT4o-Qwen2.5VL)} \\
\midrule
\textbf{GPT4o Annotation} \newline API costs (OpenAI) 
& -- 
& $\sim$200 tokens $\times$ 10 / 1M = 0.002/image. Total = 50,000 $\times$ 0.002 = \textbf{\$100} 
& Same as left $\rightarrow$ \textbf{\$100} \\

\textbf{GPT4o CoT Criticism} \newline API costs (OpenAI) 
& -- 
& $\sim$200 tokens $\times$ 10 / 1M = 0.002/image. Total = 50,000 $\times$ 0.002 = \textbf{\$100} 
& -- \\

\textbf{Qwen2.5VL CoT Criticism} \newline GPU rent costs (RunPod) 
& -- 
& -- 
& 8 A100 GPUs $\times$ 144 hrs $\times$ \$1.74/hr $\approx$ \textbf{\$2000} \\

\textbf{Human Annotation / Correction} \newline Human costs (AWS avg.) 
& 50,000 images $\times$ \$0.08 = \textbf{\$4000} 
& 10\% $\times$ 50,000 = 5,000 images $\newline \rightarrow$ 5,000 $\times$ \$0.08 = \textbf{\$400} 
& Same as left $\rightarrow$ \textbf{\$400} \\

\textbf{Total Costs} 
& \textbf{\$4000} 
& \textbf{\$600} 
& \textbf{\$2500} \\
\bottomrule
\end{tabular}}
\end{table}


\clearpage

\subsection{Extend ACT to More Complex Tasks}

For tasks where the notion of ``correct'' and ``incorrect'' becomes subjective, the criticizer can output a continuous quality score or a relative ranking rather than a binary error probability.

The criticizer can leverage a strong evaluator, e.g., an MLLM‑based evaluator or a reward model, to detect semantic inconsistencies, factual mistakes, or language issues in each candidate output and return a numerical score or rank.

For content‑dense tasks such as multi‑fact text summarisation, we can first segment the summary into individual factual statements and then evaluate each statement separately. This allows human to focus only on the segments flagged as uncertain, rather than re‑checking the entire summary.


\subsection{Ethical Considerations}
A potential ethical consideration of ACT lies in its influence on traditional annotation jobs, as the reduction of human effort could be perceived as a threat to existing human roles. However, the primary motivation of ACT is to alleviate the scalability limitations inherent in fully manual annotation, rather than to replace human annotators. By design, ACT facilitates human–AI collaboration, assigning human oversight to high-risk or ambiguous cases where nuanced judgment is essential. Importantly, this approach may also help mitigate the psychological burden associated with labeling harmful or sensitive content (e.g., depictions of violence or nudity), since human intervention is required only for a limited subset of critical instances. 
